Finding Paths for Explainable MOOC Recommendation: A Learner Perspective

The increasing availability of Massive Open Online Courses (MOOCs) has created a necessity for personalized course recommendation systems. These systems often combine neural networks with Knowledge Graphs (KGs) to achieve richer representations of learners and courses. While these enriched representations allow more accurate and personalized recommendations, explainability remains a significant challenge which is especially problematic for certain domains with significant impact such as education and online learning. Recently, a novel class of recommender systems that uses reinforcement learning and graph reasoning over KGs has been proposed to generate explainable recommendations in the form of paths over a KG. Despite their accuracy and interpretability on e-commerce datasets, these approaches have scarcely been applied to the educational domain and their use in practice has not been studied. In this work, we propose an explainable recommendation system for MOOCs that uses graph reasoning. To validate the practical implications of our approach, we conducted a user study examining user perceptions of our new explainable recommendations. We demonstrate the generalizability of our approach by conducting experiments on two educational datasets: COCO and Xuetang.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> rebuttal.tex <==
We wish to thank all the reviewers for their constructive feedback, which has provided us with the opportunity to improve the quality and impact of our work. Reviewers stated favorable opinions, noting "some interesting aspects to the paper" [R1], that "the paper is well written" [R2], and that the fact that "both an empirical and qualitative evaluation approach" is "standing out" [R3]. In the following, we respond to each reviewer in detail.

Response to Reviewer 1:
We acknowledge the insight concerning the potential for recommendations to enhance motivation and persistence within MOOC environments addressed by Reviewer 1. We will revise the introduction to integrate the papers: 
- https://doi.org/10.3991/ijep.v12i5.30523 illustrates how recommender systems can support sustained learner motivation on MOOCs
- https://doi.org/10.1016/j.compedu.2022.104684 underscores the potential to enhance student motivation in flipped classroom settings using recommender systems. 
We also acknowledge that studying how our recommendations and explanations can increase students' motivation and persistence is a very interesting future path. 

Response to Reviewer 2:
We deeply appreciate the extensive input from Reviewer 2. While there were no significant concerns to address, the detailed suggestions and commentary provided are highly valued and will be incorporated into our camera-ready submission to refine and enhance each section of our paper.

Response to Reviewer 3:
We agree with Reviewer 3 on the value of utilizing an on-campus course dataset. However, large-scale on-campus course datasets are not in the public domain, which we deemed necessary to ensure the full reproducibility of our work. Since graph-reasoning models for course recommendations are new and not widespread we wanted to ensure that all quantitative results reported in our work are reproducible. In our camera-ready version, we will emphasize our commitment to open science and the reproducibility of research, and how this commitment shaped our dataset selection process. To further emphasize our agreement with the value of utilizing an on-campus course dataset, we also want to point out that we are in the process of gathering such a dataset from our institution but it is a slow process due to ethical and anonymity considerations.

==> related_work.tex <==
\section{Related work}
\label{sec:related}
% Recently, considerable research effort has been directed toward integrating Knowledge Graphs (KGs) into Recommendation Systems (RS). In the following, we discuss approaches to KG-based recommendations as well as the use of RL for KG reasoning.

recently, blablabla

\noindent \textbf{RS for MOOCs}. 

Novel online Recommendation algorithm for Massive Open Online Courses (NoR-MOOCs) | PLOS ONE~\cite{khalid2021novel}


The Winner Takes it All: Geographic Imbalance and Provider (Un)fairness in Educational Recommender Systems~\cite{10.1145/3404835.3463235}


Interplay between upsampling and regularization for provider fairness in recommender systems~\cite{10.1007/s11257-021-09294-8}


Equality of Learning Opportunity via Individual Fairness in Personalized Recommendations~\cite{marras2021}


Enabling cross-continent provider fairness in educational recommender systems - ScienceDirect~\cite{khalid2021novel}


The Effect of Algorithmic Bias on Recommender Systems for Massive Open Online Courses~\cite{marras2019}



\noindent \textbf{Path-Based Approaches for explainable RS}. 
In contrast to embedding-based methods, path-based methods exploit paths within KGs to generate recommendations, explanations, or both. 
An approach known as CFKG~\cite{DBLP:journals/algorithms/AiACZ18} constructs a path for the explanation that originates from a user and ends at a recommended item.
This method generates an explanation after the item has been retrieved, utilizing a post hoc explanation method. 
SPrank~\cite{ostuni2013top}, another technique, extracts ontological knowledge of items and introduces an algorithm that generates semantic path-based vector features.
Another noteworthy method employs first-order logic rules to leverage KGs, extracting recommendations from the graph and then employing the Personalized PageRank algorithm to rank the recommendations~\cite{catherine2017explainable}. 
Similarly, RuleRec~\cite{ma2019jointly} introduces a learning framework for inducing explainable rules from knowledge graphs using a random-walk-based algorithm. 
The rules extracted are then used to infer associations between new items, recommend items, and explain the recommendations.
Finally, the KPRN~\cite{wang2019explainable} model learns path semantics and subsequently predicts the interaction score for the target item. 
While this model recognizes sequential dependencies between the entities on the path, it outputs all potential paths from the user to the target item.
In recent studies, utilizing RL as a method for KG reasoning has shown promising results.
The objective of RL is to learn a policy that maximizes the expected reward the agent receives when following paths in the KG.
MINERVA~\cite{das2017go}, employs RL to learn relational paths in the KG. 
This approach defines the path-finding problem as a sequential decision-making task. It employs a policy-gradient method~\cite{DBLP:journals/ml/Williams92} to discover predictive paths in response to specified queries.
Another technique called DeepPath~\cite{xiong2017deeppath} applies RL over KGs to address query-answering tasks.
ReMR~\cite{multi-level-reasoning} introduces multi-level recommendation reasoning over KGs, merging instance-view KG and ontology-view KG. 
This multi-level reasoning path approach asserts to better mimic human reasoning and enhances both the accuracy and explainability of recommendations. 
Another strategy, known as Policy-Guided Path Reasoning (PGPR)~\cite{Xian_2019}, recommends items to users based on their prior interactions with items and offers explanations for the recommendations by providing paths in KG from users to items.
While Ekar~\cite{song2019ekar} also provides paths in KG, it distinguishes itself from PGPR by considering the complete path history for training the agent and utilizing a state-of-the-art KG embedding model for reward shaping. 
Another study identifies the intentions of human dialogue and provides an interpretable path in the KG that elucidates how the intention was deduced~\cite{dialogue_mining}.
To the best of our knowledge, PGPR stands as the sole RL approach for KG reasoning that offers explainable recommendations and has an available implementation. Our work therefore builds upon the foundation laid by PGPR.


\noindent \textbf{Path-Based Approaches for explainable RS in MOOCs}. 

Reinforced Explainable Knowledge Concept Recommendation in MOOCs~\cite{10.1145/3579991}. Problems, not on public datasets, no user study, study the impact of path length only up to 3.
Towards Explainable Educational Recommendation through Path Reasoning Methods~\cite{DBLP:conf/iir/AfreenBBFM23} Dicussion paper


% The principal goal of embedding-based methods is to enhance the performance of RS by utilizing KGs to enrich item representations. 
% Collaborative Knowledge Base Embedding (CKE)~\cite{zhang2016collaborative} is a state-of-the-art method that uses TransR~\cite{Lin_Liu_Sun_Liu_Zhu_2015} graph embeddings. 
% These embeddings are then integrated into the item vector, which is designed to enhance the performance of collaborative filtering methods. 
% Ripplenet~\cite{wang2018ripplenet} extends users' interests iteratively along the KG relations to uncover their preferences.  
% \noindent \textbf{Embedding-Based Methods for RS}. The principal goal of embedding-based methods is to enhance the performance of RS by utilizing KGs to enrich item representations. 
% Collaborative Knowledge Base Embedding (CKE)~\cite{zhang2016collaborative} is a state-of-the-art method that uses TransR~\cite{Lin_Liu_Sun_Liu_Zhu_2015} graph embeddings. 
% These embeddings are then integrated into the item vector, which is designed to enhance the performance of collaborative filtering methods. 
% Ripplenet~\cite{wang2018ripplenet} extends users' interests iteratively along the KG relations to uncover their preferences.  

% \noindent \textbf{Path-Based Approaches for RS}. 
% In contrast to embedding-based methods, path-based methods exploit paths within KGs to generate recommendations, explanations, or both. 
% An approach known as CFKG~\cite{DBLP:journals/algorithms/AiACZ18} constructs a path for the explanation that originates from a user and ends at a recommended item.
% This method generates an explanation after the item has been retrieved, utilizing a post hoc explanation method. 
% SPrank~\cite{ostuni2013top}, another technique, extracts ontological knowledge of items and introduces an algorithm that generates semantic path-based vector features.
% Another noteworthy method employs first-order logic rules to leverage KGs, extracting recommendations from the graph and then employing the Personalized PageRank algorithm to rank the recommendations~\cite{catherine2017explainable}. 
% Similarly, RuleRec~\cite{ma2019jointly} introduces a learning framework for inducing explainable rules from knowledge graphs using a random-walk-based algorithm. 
% The rules extracted are then used to infer associations between new items, recommend items, and explain the recommendations.
% Finally, the KPRN~\cite{wang2019explainable} model learns path semantics and subsequently predicts the interaction score for the target item. 
% While this model recognizes sequential dependencies between the entities on the path, it outputs all potential paths from the user to the target item.

% \noindent \textbf{RL for KG reasoning}. 
% In recent studies, utilizing RL as a method for KG reasoning has shown promising results.
% The objective of RL is to learn a policy that maximizes the expected reward the agent receives when following paths in the KG.
% MINERVA~\cite{das2017go}, employs RL to learn relational paths in the KG. 
% This approach defines the path-finding problem as a sequential decision-making task. It employs a policy-gradient method~\cite{DBLP:journals/ml/Williams92} to discover predictive paths in response to specified queries.
% Another technique called DeepPath~\cite{xiong2017deeppath} applies RL over KGs to address query-answering tasks.
% ReMR~\cite{multi-level-reasoning} introduces multi-level recommendation reasoning over KGs, merging instance-view KG and ontology-view KG. 
% This multi-level reasoning path approach asserts to better mimic human reasoning and enhances both the accuracy and explainability of recommendations. 
% Another strategy, known as Policy-Guided Path Reasoning (PGPR)~\cite{Xian_2019}, recommends items to users based on their prior interactions with items and offers explanations for the recommendations by providing paths in KG from users to items.
% While Ekar~\cite{song2019ekar} also provides paths in KG, it distinguishes itself from PGPR by considering the complete path history for training the agent and utilizing a state-of-the-art KG embedding model for reward shaping. 
% Another study identifies the intentions of human dialogue and provides an interpretable path in the KG that elucidates how the intention was deduced~\cite{dialogue_mining}.
% To the best of our knowledge, PGPR stands as the sole RL approach for KG reasoning that offers explainable recommendations and has an available implementation. Our work therefore builds upon the foundation laid by PGPR.
